Release Sooner, Expose Less: Offloading MoE Dispatch in NCCL-EP under Dual-Batch Overlap

Dual-batch overlap (DBO) hides mixture-of-experts (MoE) communication behind another microbatch's computation, but only after dispatch send releases the GPU. The time dispatch send holds the GPU therefore stays exposed, while network progress after release can be hidden. We evaluate GPUDirect Async - Kernel Initiated (GDA-KI) Free Flow, an NCCL-EP research configuration that leaves WQE construction on the GPU but moves send progression to a host thread. On a GB300 NVL72 system, GDA-KI Free Flow reduces dispatch-send time relative to default GDA-KI at every operating point in the evaluated parameter sweep. An experiment that inserts a GPU delay between dispatch send and receive shows that offload increases the in-flight interval. Depending on the load, 32-96 microseconds of computation or other independent work between send and receive hides the deferred progress, leaving less exposed time than default GDA-KI. In disaggregated vLLM serving with DBO, GDA-KI Free Flow lowers median TPOT by 15-25% relative to NCCL-EP default GDA-KI and by 16-42% relative to DeepEP v1.

==> figures/serving_tpot.tex <==
\begin{tikzpicture}
\begin{axis}[
  width=\servingplotwidth,
  height=0.20\textwidth,
  scale only axis,
  symbolic x coords={128,256,512,1000},
  xmin=128,xmax=1000,
  ymin=11.5,ymax=23.5,
  xtick={128,256,512,1000},
  ytick={12,14,16,18,20,22},
  xlabel={client concurrency},
  ylabel={median TPOT (ms)},
  label style={font=\scriptsize},
  tick label style={font=\scriptsize},
  grid=major,
  legend columns=3,
  legend style={
    font=\scriptsize,
    draw=none,
    at={(0.5,1.02)},
    anchor=south,
    /tikz/column 2/.style={column sep=3pt},
  },
]

\addplot[color=gdakicolor,mark=square*,very thick]
  table[col sep=comma,x=c,y=gdaki]
  {figures/data/serving_tpot_high_concurrency.csv};
\addlegendentry{NCCL-EP baseline}

\addplot[color=deepepcolor,mark=pentagon*,very thick,dashed]
  table[col sep=comma,x=c,y=deepep_gdaki]
  {figures/data/serving_tpot_high_concurrency.csv};
\addlegendentry{DeepEP baseline}

\addplot[color=freeflowcolor,mark=diamond*,very thick]
  table[col sep=comma,x=c,y=gdaki_free_flow]
  {figures/data/serving_tpot_high_concurrency.csv};
\addlegendentry{GDA-KI Free Flow}
\end{axis}
\end{tikzpicture}

